Matching-space Stereo Networks for Cross-domain Generalization

End-to-end deep networks represent the state of the art for stereo matching. While excelling on images framing environments similar to the training set, major drops in accuracy occur in unseen domains (e.g., when moving from synthetic to real scenes). In this paper we introduce a novel family of architectures, namely Matching-Space Networks (MS-Nets), with improved generalization properties. By replacing learning-based feature extraction from image RGB values with matching functions and confidence measures from conventional wisdom, we move the learning process from the color space to the Matching Space, avoiding over-specialization to domain specific features. Extensive experimental results on four real datasets highlight that our proposal leads to superior generalization to unseen environments over conventional deep architectures, keeping accuracy on the source domain almost unaltered. Our code is available at https://github.com/ccj5351/MS-Nets.

==> comments.tex <==
\matteo{
\noindent More titles:
\begin{enumerate}
\item Robust networks for in-the-wild stereo matching
\item Matching space stereo networks for cross-domain generalization
\end{enumerate}
More comments:
\begin{enumerate}
\item Probably, CBMV-style makes the paper \textit{incremental}. What about using a more vague name, maybe referring to matching space versus color space? Then, we will say that we choose cbmv features because ...
\item Same for the networks. CBMV-GCNet may drive the reviewers to think that it is just CBMV + GCNet 
\item (form) tables 2-4 are small now, we may consider to bring some of them on two rows 
\item I don't know if we need more qualitatives. Fig.1 seems pretty strong to me 
\item Table 2, most entries where from https://arxiv.org/pdf/1903.01700.pdf, Table 12 (now accepted). The numbers are now different, we should fix. CBMV-GCNet is still the winner. 
\item Table 2, I would add https://arxiv.org/pdf/1911.13287.pdf, either if accepted to CVPR or not. Numbers are 6.2 and 6.5 from their Table 3, CBMV-GCNet is better. Since they are based on GANet, I think it would be nice to show that we are better.
\item R3 at CVPR asked for intermediate representations (feature maps or cost volumes, he explained in the final review). Maybe we can show the final cost volume before soft-argmax operator from traditional and CBMV networks. I remember a nice visualization tool by Kostas in the original CBMV paper...
\end{enumerate}

}

\PMcomments{
Title: I think that generalization should be in the title. The rest can be changed. For example, we don't need to specify that it's about 3D architectures.

1. Matching space makes sense. We'll have to talk representations being the most important thing for AI and vision. I agree.

2. I'm OK with dropping CBMV as a pre-fix, but we should come up with another prefix because if the various networks don't have clear names, the paper will be very confusing.

6. CVPR 2020 are not prior art for ECCV. 

7. Intermediate representations make no sense in end-to-end systems. This was an unfounded comment that I don't think we should address. What is a meaningful intermediate result? See the Zbontar JMLR paper, for example, that provides evidence how intermediate high accuracies (e.g. NCC vs census) don't lead to high final accuracy.

CVPR reviews: I believe that we addressed them reasonably well in the rebuttal.

}

